A Sub-Nyquist Radar Prototype: Hardware and Algorithms

Traditional radar sensing typically involves matched filtering between the received signal and the shape of the transmitted pulse. Under the confinement of classic sampling theorem this requires that the received signals must first be sampled at twice the baseband bandwidth, in order to avoid aliasing. The growing demands for target distinction capability and spatial resolution imply significant growth in the bandwidth of the transmitted pulse. Thus, correlation based radar systems require high sampling rates, and with the large amounts of data sampled also necessitate vast memory capacity. In addition, real-time processing of the data typically results in high power consumption. Recently, new approaches for radar sensing and detection were introduced, based on the Finite Rate of Innovation and Xampling frameworks. These techniques allow significant reduction in sampling rate, implying potential power savings, while maintaining the system's detection capabilities at high enough SNR. Here we present for the first time a design and implementation of a Xampling-based hardware prototype that allows sampling of radar signals at rates much lower than Nyquist. We demostrate by real-time analog experiments that our system is able to maintain reasonable detection capabilities, while sampling radar signals that require sampling at a rate of about 30MHz at a total rate of 1Mhz.

==> citations.tex <==
@article{Shannon,
    author = {Shannon, C. E.},
    doi = {10.1109/JRPROC.1949.232969},
    issn = {0096-8390},
    journal = {Proceedings of the IRE},
    number = {1},
    pages = {10--21},
    posted-at = {2008-12-10 19:01:03},
    priority = {2},
    title = {{Communication in the Presence of Noise}},
    url = {http://dx.doi.org/10.1109/JRPROC.1949.232969},
    volume = {37},
    year = {1949}
}

@ARTICLE{Cook,
author={Cook, C. E.},
journal={Proceedings of the IRE}, title={Pulse Compression-Key to More Efficient Radar Transmission},
year={1960},
volume={48},
number={3},
pages={310--316},
doi={10.1109/JRPROC.1960.287599},
ISSN={0096-8390},}

@ARTICLE{Sarkar,
author={Sarkar, T. K. and Pereira, O.},
journal={Antennas and Propagation Magazine, IEEE}, title={Using the matrix pencil method to estimate the parameters of a sum of complex exponentials},
year={1995},
volume={37},
number={1},
pages={48--55},
doi={10.1109/74.370583},
ISSN={1045-9243},}

@book{StoicaMoses,
    author = {Stoica, P. and Moses, R.L.},
    day = {06},
    howpublished = {Paperback},
    isbn = {0132584190},
    keywords = {coherence, signal\_processing, spectral\_analysis},
    posted-at = {2007-10-22 14:09:41},
    priority = {2},
    publisher = {{Prentice Hall}},
    title = {{Introduction to Spectral Analysis}},
    year = {1997}
}

@incollection{Vershynin,
    author = {Vershynin, R.},
    booktitle = {{Compressed Sensing: Theory and Applications}},
    publisher = {{Cambridge University Press}},
    title = {{Introduction to the non-asymptotic analysis of random metrices}}
    chapter={5},
    editor = {Y. C. Eldar and G. Kutyniok},
    pages={210--268},
    year = {2012}
}

@ARTICLE{Duarte,
author={Duarte, M.F. and Eldar, Y.C.},
journal={Signal Processing, IEEE Transactions on},
title={Structured Compressed Sensing: From Theory to Applications},
year={2011},
volume={59},
number={9},
pages={4053-4085},

}

@ARTICLE{Vetterli,
author={Vetterli, M. and Marziliano, P. and Blu, T.},
journal={Signal Processing, IEEE Trans. on},
title={Sampling signals with finite rate of innovation},
year={2002},
volume={50},
number={6},
pages={1417--1428},
doi={10.1109/TSP.2002.1003065},
ISSN={1053-587X},}

@ARTICLE{Tropp,
author={Tropp, J. A. and Gilbert, A. C.},
journal={Information Theory, IEEE Trans. on}, title={Signal Recovery From Random Measurements Via Orthogonal Matching Pursuit},
year={2007},
volume={53},
number={12},
pages={4655--4666},
doi={10.1109/TIT.2007.909108},
ISSN={0018-9448},}

@INPROCEEDINGS{Rudelson,
author={Rudelson, M. and Vershynin, R.},
booktitle={Information Sciences and Systems, 2006 40th Annual Conference on},
title={Sparse reconstruction by convex relaxation: Fourier and Gaussian measurements},
year={2006},
volume={},
number={},
pages={207--212},
doi={10.1109/CISS.2006.286463},
ISSN={},}

@ARTICLE{OMP,
  author =       {Stephane G. Mallat and Zhifeng Zhang},
  title =        {{Matching Pursuits with Time-Frequency Dictionaries}},
  journal =      {IEEE Trans. Signal Process.},
  year =         {1993},
  volume =       {41},
  number =       {12},
  pages =        {3397--3415},
  month =        {Dec.},
}

@ARTICLE{BE13,
author={O. Bar-Ilan and Y. C. Eldar},
note={submitted to {\em IEEE Trans. Signal Processing}},
title={Sub-Nyquist Radar via Doppler Focusing},
year={2013},
}

@ARTICLE{Tur,
author={Tur, R. and Eldar, Y. C. and Friedman, Z.},
journal={Signal Processing, IEEE Trans. on}, title={Innovation Rate Sampling of Pulse Streams With Application to Ultrasound Imaging},
year={2011},
volume={59},
number={4},
pages={1827--1842},
doi={10.1109/TSP.2011.2105480},
ISSN={1053-587X},}

@ARTICLE{Mishali1,
author={Mishali, M. and Eldar, Y. C. and Elron, E.},
journal={Signal Processing, IEEE Trans. on}, title={Xampling: Signal Acquisition and Processing in Union of Subspaces},
year={2011},
volume={59},
number={10},
pages={4719--4734},
}

@ARTICLE{Bajwa,
author={Bajwa, W. U. and Gedalyahu, K. and Eldar, Y. C.},
journal={Signal Processing, IEEE Trans. on}, title={Identification of Parametric Underspread Linear Systems and Super-Resolution Radar},
year={2011},
volume={59},
number={6},
pages={2548--2561},
doi={10.1109/TSP.2011.2114657},
ISSN={1053-587X},}

@ARTICLE{Gedal,
author={Gedalyahu, K. and Tur, R. and Eldar, Y.C.},
journal={Signal Processing, IEEE Trans. on}, title={Multichannel Sampling of Pulse Streams at the Rate of Innovation},
year={2011},
volume={59},
number={4},
pages={1491--1504},
ISSN={1053-587X},}

@ARTICLE{Stoica,
author={Stoica, P. and Babu, P.},
journal={Signal Processing, IEEE Trans. on}, title={Sparse Estimation of Spectral Lines: Grid Selection Problems and Their Solutions},
year={2012},
volume={60},
number={2},
pages={962--967},
doi={10.1109/TSP.2011.2175222},
ISSN={1053-587X},}

@book{Eldar,
    author = {Eldar, Y. C. and Kutyniok, G.},
    howpublished = {Hardcover},
    publisher = {{Cambridge University Press}},
    title = {{Compressed Sensing: Theory and Applications}},
    editor = "Y. C. Eldar and G. Kutyniok",
    year = {2012}
}



@ARTICLE{Herman,
author={Herman, M.A. and Strohmer, T.},
journal={Signal Processing, IEEE Transactions on},
title={High-Resolution Radar via Compressed Sensing},
year={2009},
volume={57},
number={6},
pages={2275-2284},
}

@INPROCEEDINGS{Anitori,
author={Anitori, L. and Otten, M. and Hoogeboom, P.},
booktitle={Microwave Conference Proceedings (APMC), 2010 Asia-Pacific},
title={Compressive sensing for high resolution radar imaging},
year={2010},
pages={1809-1812},
}


@ARTICLE{Wagner,
author={Wagner, N. and Eldar, Y. C. and Friedman, Z.},
journal={accepted Signal Processing, IEEE Trans. on},
title={Compressed Beamforming in Ultrasound Imaging},
year={2012},
}

@ARTICLE{Friis,
author = {Friis, H. T.},
title = {Noise figures of radio receivers}, 	
journal = {Proceedings of the IRE},
volume = {32},
pages ={419--422},
year= {1944},}

@ARTICLE{Mishali,
author = {Mishali, M. and Eldar, Y. C. and Dounaevsky, O.  and Shoshan, E.},
title = {Xampling: Analog to Digital at Sub-Nyquist Rates}, 	
journal = {IET Journal of Circuits, Devices and Systems},
volume = {5, Issue 1},
pages ={8--20},
year= {2011},}

@article{Wagner,
  author    = {Noam Wagner and Yonina C. Eldar and Zvi Friedman},
  title     = {{Compressed Beamforming in Ultrasound Imaging}},
  journal   = {IEEE Trans. Signal Process.},
  volume    = {60},
  number    = {9},
  month     = {Sep.},
  pages     = {4643--4657},
  year      = {2012},
}

@ARTICLE{CandesCSIntro,
  author =       {E. J. Candes and M. B. Wakin},
  title =        {{An Introduction to Compressive Sampling}},
  journal =      {IEEE Signal Processing Magazine},
  year =         {2008},
  volume =       {25},
  number =       {2},
  pages =        {21--30},
  month =        {Mar.},
}

@ARTICLE{BlockSparse,
  author =       {B. Demissie},
  title =        {{High-Resolution Range-Doppler Imaging by Coherent Block-Sparse Estimation}},
  journal =      {International Workshop on Compressed Sensing Applied to Radar},
  year =         {2012},
  month =        {May},
}

@ARTICLE{AdaptiveCSRadar,
  author =       {J. Zhang and D. Zhu and G. Zhang},
  title =        {{Adaptive Compressed Sensing Radar Oriented Toward Cognitive Detection in Dynamic Sparse Target Scene}},
  journal =      {IEEE Trans. Signal Process.},
  year =         {2012},
  volume =       {60},
  number =       {4},
  pages =        {1718--1729},
  month =        {Apr.},
}

@conference {CompressiveRadarImaging,
	title = {{Compressive Radar Imaging}},
	booktitle = {IEEE Radar Conference},
	year = {2007},
	month = {Apr.},
	address = {Waltham, MA},
	author = {Richard G. Baraniuk and Steeghs, Philippe}
}

@BOOK{Richards,
  author =       {Mark A. Richards},
  title =        {{Fundamentals of Radar Signal Processing}},
  publisher =    {McGraw Hill, New York, NY},
  year =         {2005},
}

@ARTICLE{MUSIC,
  author =       {R. Schmidt},
  title =        {{Multiple Emitter Location and Signal Parameter Estimation}},
  journal =      {IEEE Trans. Antennas Propag.},
  volume =       {34},
  number =       {3},
  year =         {1986},
  pages =        {276=-280},
  month =        {Mar.},
}
